Non-standard interactions and the CP phase measurements in neutrino oscillations at low energies

We study the effects of non-standard interactions (NSI) and the genuine CP phase $\delta_D$ in neutrino oscillations at low, $E_\nu \lesssim 1\,\mbox{GeV}$, and very low, $E_\nu \lesssim 0.1\,\mbox{GeV}$, energies. For experimental setup with baseline and neutrino energy tuned to the first 1-3 oscillation maximum, we develop a simple analytic formalism to show the effects of NSI. The vacuum mimicking and its violation as well as the use of the separation basis play a central role in our formalism. The NSI corrections that affect the CP phase measurement mainly come from the violation of vacuum mimicking as well as from the corrections to the 1-3 mixing angle and mass-squared difference. We find that the total NSI correction to the $\nu_\mu - \nu_e$ probability $P_{\mu e}$ can reach $20\% - 30\%$ ($1 \sigma$) at T2(H)K. Correspondingly, the correction to the CP phase can be as large as $50^\circ$ and hence significantly deteriorates the CP sensitivity at T2(H)K. The proposed TNT2K experiment, a combination of T2(H)K and the short baseline experiment $\mu$Kam that uses the Super-K/Hyper-K detector at Kamioka to measure the oscillation of the antineutrinos from muon decay at rest ($\mu$DAR), can substantially reduce the degeneracy between NSI and the genuine CP phase $\delta_D$ to provide high CP sensitivity. The NSI correction to $P_{\mu e}$ is only $2\%$ ($1 \sigma$) for $\mu$DAR neutrinos.

==> Makefile <==
#
# Makefile for nuMatter
#
# Shao-Feng Ge (gesf02@gmail.com) 
# 
# created on Mon Jun 20 22:45:34 CEST 2016
#

# record
record:
	uname -a > record.log
	echo >> record.log
	echo $(PWD) >> record.log
	echo >> record.log
	date >> record.log

# backup [time stamp according to the newest file]
figures=\
code/nuNSI_*_Pme.eps \
code/nuNSI_*_Pme_ASI.eps \
code/muDAR.eps \
code/T2K.eps \
code/nuNSI_*_??_rVacuum.eps \
code/nuNSI_*_??_tdCP.eps \
code/nuNSI_*_??_fPme.eps \
code/nuNSI_*_??_dPme0.eps \
code/nuNSI_*_E?_dPme4rV.eps \
code/nuNSI_*_E?_dPme4dD.eps \
code/nuNSI_dCP_error4_new_T2K_prior.eps \
code/nuNSI_dCP_error4_muSK.eps \
code/nuNSI_dCP_error4_new_T2K_muSK_prior.eps \
code/nuNSI_dCP_error4_new_nuT2K_muSK_prior.eps

# backup
backupFiles= nuMatter.tex nuMatter.bib nuMatter.bbl Makefile $(figures)
backup: record
	tar czvf nuMatter_$(shell date -r $(shell ls -t $(backupFiles) | head -1) +'%y%m%d_%H%M%S').tgz $(backupFiles) record.log

# submission
submissionFiles= nuMatter.tex nuMatter.bbl $(figures)
submission: record
	tar czvf nuMatter_submission_$(shell date -r $(shell ls -t $(backupFiles) | head -1) +'%y%m%d_%H%M%S').tar.gz $(submissionFiles)

# plots
plots:
	tar czvf nuMatter_figs_$(shell date -r $(shell ls -t $(figures) | head -1) +'%y%m%d_%H%M%S').tgz $(figures)

